Comparisons of eccentric binary black hole simulations with post-Newtonian models

We present the first comparison between numerical relativity (NR) simulations of an eccentric binary black hole system with corresponding post-Newtonian (PN) results. We evolve an equal-mass, non-spinning configuration with an initial eccentricity e ~ 0.1 for 21 gravitational wave cycles before merger, and find agreement in the gravitational wave phase with an adiabatic eccentric PN model with 2 PN radiation reaction within 0.1 radians for 10 cycles. The NR and PN phase difference grows to 0.7 radians by 5 cycles before merger. We find that these results can be obtained by expanding the eccentric PN expressions in terms of the frequency-related variable x = (omega M)^{2/3} with M the total mass of the binary. When using instead the mean motion n = 2 \pi /P, where P is the orbital period, the comparison leads to significant disagreements with NR.

==> include/eDot-1.tex <==
(93184 \eta -125361) e^4+12 (54271 \eta -59834) e^2+8 (28588 \eta +8451)

==> include/eDot-2b.tex <==
\big(2758560 \eta ^2-4344852 \eta +3786543\big) e^6+\big(42810096 \eta ^2-78112266 \eta +46579718\big) e^4+\big(48711348 \eta ^2-35583228 \eta -36993396\big) e^2+4548096 \eta ^2+\sqrt{1-e^2} \big((2847600-1139040 \eta ) e^4+(35093520-14037408 \eta ) e^2-5386752 \eta +13466880\big)+13509360 \eta -15198032

==> include/eph-3b.tex <==
\big(13440 \eta ^2+483840 \eta -940800\big) e^4+\big(255360 \eta ^2+17220 \pi ^2 \eta -2880640 \eta +2688000\big) e^2-268800 \eta ^2+2396800 \eta +\sqrt{1-e^2} \big(\big(1050 \eta ^3-134050 \eta ^2+786310 \eta -860160\big) e^4+\big(-18900 \eta ^3+553980 \eta ^2+4305 \pi ^2 \eta -1246368 \eta +2042880\big) e^2+276640 \eta ^2+2674480 \eta -17220 \eta  \pi ^2-1451520\big)-17220 \eta  \pi ^2-1747200

==> include/kappaE.tex <==
\sum _{p=1}^{\infty } \frac{1}{4} p^3 \big(\big(\big(-e^2-\frac{3}{e^2}+\frac{1}{e^4}+3\big) p^2+\frac{1}{3}-\frac{1}{e^2}+\frac{1}{e^4}\big) J_p(p e){}^2+\big(-3 e-\frac{4}{e^3}+\frac{7}{e}\big) p J_p'(p e) J_p(p e)+\big(\big(e^2+\frac{1}{e^2}-2\big) p^2+\frac{1}{e^2}-1\big) J_p'(p e){}^2\big)

==> include/l-3.tex <==
35 \big(96 \big(11 \eta ^2-29 \eta +30\big) e^2+960 \eta ^2+\eta  \big(-13184+123 \pi ^2\big)+8640\big) (u-v) (e \cos (u)-1)^3+3360 \big(-12 (2 \eta -5) (u-v)+12 e (2 \eta -5) \cos (u) (u-v)+e \sqrt{1-e^2} (\eta -15) \eta  \sin (u)\big) (e \cos (u)-1)^2+e \sqrt{1-e^2} \big(140 \big(13 e^4-11 e^2-2\big) \eta ^3-140 \big(73 e^4-325 e^2+444\big) \eta ^2+\big(3220 e^4-148960 e^2-4305 \pi ^2+143868\big) \eta +e^2 \big(1820 \big(e^2-1\big) \eta ^3-140 \big(83 e^2+109\big) \eta ^2-\big(1120 e^2+4305 \pi ^2+752\big) \eta +67200\big) \cos ^2(u)-2 e \big(1960 \big(e^2-1\big) \eta ^3+6720 \big(e^2-5\big) \eta ^2+\big(-71820 e^2-4305 \pi ^2+69948\big) \eta +67200\big) \cos (u)+67200\big) \sin (u)

==> include/n-3.tex <==
(1536 \eta -3840) e^4+(1920-768 \eta ) e^2-768 \eta +\sqrt{1-e^2} \big(\big(1040 \eta ^2-1760 \eta +2496\big) e^4+\big(5120 \eta ^2+123 \pi ^2 \eta -17856 \eta +8544\big) e^2+896 \eta ^2-14624 \eta +492 \eta  \pi ^2-192\big)+1920

==> include/name.tex <==
Null


==> include/om-2.tex <==
\big(-12 \eta ^2-18 \eta \big) e^6+\big(20 \eta ^2-26 \eta -60\big) e^4+\big(-2 \eta ^2+50 \eta +75\big) e^2+\big(\big(-14 \eta ^2+8 \eta -147\big) e^5+\big(8 \eta ^2+22 \eta +42\big) e^3\big) \cos ^3(u)+\big(\big(17 \eta ^2-17 \eta +48\big) e^6+\big(-4 \eta ^2-38 \eta +153\big) e^4+\big(5 \eta ^2-35 \eta +114\big) e^2\big) \cos ^2(u)-36 \eta +\big(\big(-\eta ^2+97 \eta +12\big) e^5+\big(-16 \eta ^2-74 \eta -81\big) e^3+\big(-\eta ^2+67 \eta -246\big) e\big) \cos (u)+\sqrt{1-e^2} \big(e^3 (36 \eta -90) \cos ^3(u)+\big((180-72 \eta ) e^4+(90-36 \eta ) e^2\big) \cos ^2(u)+\big((144 \eta -360) e^3+(90-36 \eta ) e\big) \cos (u)+e^2 (180-72 \eta )+36 \eta -90\big)+90

==> include/om-3.tex <==
\big(10080 \eta ^3+40320 \eta ^2-15120 \eta \big) e^{10}+\big(-52640 \eta ^3-13440 \eta ^2+483280 \eta \big) e^8+\big(84000 \eta ^3-190400 \eta ^2-17220 \pi ^2 \eta -50048 \eta -241920\big) e^6+\big(-52640 \eta ^3+516880 \eta ^2+68880 \pi ^2 \eta -1916048 \eta +262080\big) e^4+\big(4480 \eta ^3-412160 \eta ^2-30135 \pi ^2 \eta +553008 \eta +342720\big) e^2+\big(\big(13440 \eta ^3+94640 \eta ^2-113680 \eta -221760\big) e^9+\big(-11200 \eta ^3-112000 \eta ^2+12915 \pi ^2 \eta +692928 \eta -194880\big) e^7+\big(4480 \eta ^3+8960 \eta ^2-43050 \pi ^2 \eta +1127280 \eta -147840\big) e^5\big) \cos ^5(u)+\big(\big(-16240 \eta ^3+12880 \eta ^2+18480 \eta \big) e^{10}+\big(16240 \eta ^3-91840 \eta ^2+17220 \pi ^2 \eta -652192 \eta +100800\big) e^8+\big(-55440 \eta ^3+34160 \eta ^2-30135 \pi ^2 \eta -2185040 \eta +2493120\big) e^6+\big(21840 \eta ^3+86800 \eta ^2+163590 \pi ^2 \eta -5713888 \eta +228480\big) e^4\big) \cos ^4(u)+\big(\big(560 \eta ^3-137200 \eta ^2+388640 \eta +241920\big) e^9+\big(30800 \eta ^3-264880 \eta ^2-68880 \pi ^2 \eta +624128 \eta +766080\big) e^7+\big(66640 \eta ^3+612080 \eta ^2-8610 \pi ^2 \eta +6666080 \eta -6652800\big) e^5+\big(-30800 \eta ^3-294000 \eta ^2-223860 \pi ^2 \eta +9386432 \eta \big) e^3\big) \cos ^3(u)+67200 \eta ^2+\big(\big(4480 \eta ^3-20160 \eta ^2+16800 \eta \big) e^{10}+\big(3920 \eta ^3+475440 \eta ^2-17220 \pi ^2 \eta +831952 \eta -725760\big) e^8+\big(-75600 \eta ^3+96880 \eta ^2+154980 \pi ^2 \eta -3249488 \eta -685440\big) e^6+\big(5040 \eta ^3-659120 \eta ^2+25830 \pi ^2 \eta -7356624 \eta +6948480\big) e^4+\big(-5040 \eta ^3+190960 \eta ^2+137760 \pi ^2 \eta -7307920 \eta +107520\big) e^2\big) \cos ^2(u)-761600 \eta +\big(\big(-2240 \eta ^3-168000 \eta ^2-424480 \eta \big) e^9+\big(28560 \eta ^3+242480 \eta ^2+34440 \pi ^2 \eta -1340224 \eta +725760\big) e^7+\big(-33040 \eta ^3-754880 \eta ^2-172200 \pi ^2 \eta +5458480 \eta -221760\big) e^5+\big(40880 \eta ^3+738640 \eta ^2+30135 \pi ^2 \eta +1554048 \eta -2936640\big) e^3+\big(-560 \eta ^3-100240 \eta ^2-43050 \pi ^2 \eta +3284816 \eta -389760\big) e\big) \cos (u)+\sqrt{1-e^2} \big(\big(\big(-127680 \eta ^2+544320 \eta -739200\big) e^7+\big(-53760 \eta ^2-8610 \pi ^2 \eta +674240 \eta -67200\big) e^5\big) \cos ^5(u)+\big(\big(161280 \eta ^2-477120 \eta +537600\big) e^8+\big(477120 \eta ^2+17220 \pi ^2 \eta -2894080 \eta +2217600\big) e^6+\big(268800 \eta ^2+25830 \pi ^2 \eta -2721600 \eta +1276800\big) e^4\big) \cos ^4(u)+\big(\big(-524160 \eta ^2+1122240 \eta -940800\big) e^7+\big(-873600 \eta ^2-68880 \pi ^2 \eta +7705600 \eta -3897600\big) e^5+\big(-416640 \eta ^2-17220 \pi ^2 \eta +3357760 \eta -3225600\big) e^3\big) \cos ^3(u)+\big(\big(604800 \eta ^2-504000 \eta -403200\big) e^6+\big(1034880 \eta ^2+103320 \pi ^2 \eta -11195520 \eta +5779200\big) e^4+\big(174720 \eta ^2-17220 \pi ^2 \eta -486080 \eta +2688000\big) e^2\big) \cos ^2(u)+\big(\big(-282240 \eta ^2-450240 \eta +1478400\big) e^5+\big(-719040 \eta ^2-68880 \pi ^2 \eta +8128960 \eta -5040000\big) e^3+\big(94080 \eta ^2+25830 \pi ^2 \eta -1585920 \eta -470400\big) e\big) \cos (u)-67200 \eta ^2+761600 \eta +e^4 \big(40320 \eta ^2+309120 \eta -672000\big)+e^2 \big(208320 \eta ^2+17220 \pi ^2 \eta -2289280 \eta +1680000\big)-8610 \eta  \pi ^2-201600\big)+8610 \eta  \pi ^2+201600

==> include/om-3man.tex <==
\big(10080 \eta ^3+40320 \eta ^2-15120 \eta \big) e^{10}+\big(-52640 \eta ^3-13440 \eta ^2+483280 \eta \big) e^8 \nonumber \\
& \quad +\big(84000 \eta ^3-190400 \eta ^2-17220 \pi ^2 \eta -50048 \eta -241920\big) e^6+\big(-52640 \eta ^3+516880 \eta ^2+68880 \pi ^2 \eta  \nonumber \\
& \quad -1916048 \eta +262080\big) e^4+\big(4480 \eta ^3-412160 \eta ^2-30135 \pi ^2 \eta +553008 \eta +342720\big) e^2+\big(\big(13440 \eta ^3+94640 \eta ^2 \nonumber \\
& \quad -113680 \eta -221760\big) e^9+\big(-11200 \eta ^3-112000 \eta ^2+12915 \pi ^2 \eta +692928 \eta -194880\big) e^7+\big(4480 \eta ^3+8960 \eta ^2 \nonumber \\
& \quad -43050 \pi ^2 \eta +1127280 \eta -147840\big) e^5\big) \cos ^5(u)+\big(\big(-16240 \eta ^3+12880 \eta ^2+18480 \eta \big) e^{10}+\big(16240 \eta ^3-91840 \eta ^2 \nonumber \\
& \quad +17220 \pi ^2 \eta -652192 \eta +100800\big) e^8+\big(-55440 \eta ^3+34160 \eta ^2-30135 \pi ^2 \eta -2185040 \eta +2493120\big) e^6 \nonumber \\
& \quad +\big(21840 \eta ^3+86800 \eta ^2+163590 \pi ^2 \eta -5713888 \eta +228480\big) e^4\big) \cos ^4(u)+\big(\big(560 \eta ^3-137200 \eta ^2+388640 \eta \nonumber \\
& \quad  +241920\big) e^9+\big(30800 \eta ^3-264880 \eta ^2-68880 \pi ^2 \eta +624128 \eta +766080\big) e^7+\big(66640 \eta ^3+612080 \eta ^2-8610 \pi ^2 \eta  \nonumber \\
& \quad  +6666080 \eta -6652800\big) e^5+\big(-30800 \eta ^3-294000 \eta ^2-223860 \pi ^2 \eta +9386432 \eta \big) e^3\big) \cos ^3(u)+67200 \eta ^2 \nonumber \\
& \quad +\big(\big(4480 \eta ^3-20160 \eta ^2+16800 \eta \big) e^{10}+\big(3920 \eta ^3+475440 \eta ^2-17220 \pi ^2 \eta +831952 \eta -725760\big) e^8+\big(-75600 \eta ^3 \nonumber \\
& \quad +96880 \eta ^2+154980 \pi ^2 \eta -3249488 \eta -685440\big) e^6+\big(5040 \eta ^3-659120 \eta ^2+25830 \pi ^2 \eta -7356624 \eta +6948480\big) e^4 \nonumber
\end{align}

\begin{align}
& \quad +\big(-5040 \eta ^3+190960 \eta ^2+137760 \pi ^2 \eta -7307920 \eta +107520\big) e^2\big) \cos ^2(u)-761600 \eta +\big(\big(-2240 \eta ^3-168000 \eta ^2 \nonumber \\
& \quad -424480 \eta \big) e^9+\big(28560 \eta ^3+242480 \eta ^2+34440 \pi ^2 \eta -1340224 \eta +725760\big) e^7+\big(-33040 \eta ^3-754880 \eta ^2 \nonumber \\
& \quad -172200 \pi ^2 \eta +5458480 \eta -221760\big) e^5+\big(40880 \eta ^3+738640 \eta ^2+30135 \pi ^2 \eta +1554048 \eta -2936640\big) e^3 \nonumber \\
& \quad +\big(-560 \eta ^3-100240 \eta ^2-43050 \pi ^2 \eta +3284816 \eta -389760\big) e\big) \cos (u)+\sqrt{1-e^2} \big(\big(\big(-127680 \eta ^2+544320 \eta  \nonumber \\
& \quad -739200\big) e^7+\big(-53760 \eta ^2-8610 \pi ^2 \eta +674240 \eta -67200\big) e^5\big) \cos ^5(u)+\big(\big(161280 \eta ^2-477120 \eta +537600\big) e^8 \nonumber \\
& \quad +\big(477120 \eta ^2+17220 \pi ^2 \eta -2894080 \eta +2217600\big) e^6+\big(268800 \eta ^2+25830 \pi ^2 \eta -2721600 \eta  \nonumber \\
& \quad +1276800\big) e^4\big) \cos ^4(u)+\big(\big(-524160 \eta ^2+1122240 \eta -940800\big) e^7+\big(-873600 \eta ^2-68880 \pi ^2 \eta +7705600 \eta  \nonumber \\
& \quad -3897600\big) e^5+\big(-416640 \eta ^2-17220 \pi ^2 \eta +3357760 \eta -3225600\big) e^3\big) \cos ^3(u)+\big(\big(604800 \eta ^2-504000 \eta \nonumber \\
& \quad  -403200\big) e^6+\big(1034880 \eta ^2+103320 \pi ^2 \eta -11195520 \eta +5779200\big) e^4+\big(174720 \eta ^2-17220 \pi ^2 \eta -486080 \eta  \nonumber \\
& \quad +2688000\big) e^2\big) \cos ^2(u)+\big(\big(-282240 \eta ^2-450240 \eta +1478400\big) e^5+\big(-719040 \eta ^2-68880 \pi ^2 \eta +8128960 \eta   \nonumber \\
& \quad  -5040000\big) e^3+\big(94080 \eta ^2+25830 \pi ^2 \eta -1585920 \eta -470400\big) e\big) \cos (u)-67200 \eta ^2+761600 \eta +e^4 \big(40320 \eta ^2  \nonumber \\
& \quad +309120 \eta -672000\big)+e^2 \big(208320 \eta ^2+17220 \pi ^2 \eta -2289280 \eta +1680000\big)-8610 \eta  \pi ^2 -201600\big)+8610 \eta  \pi ^2 \nonumber \\
& \quad+201600

==> include/radius-2d.tex <==
\sqrt{1-e^2} \left(\frac{1}{72} (180-72 \eta ) \cos (u) e^3+\frac{1}{72} \
(360-144 \eta ) e^2+\frac{1}{72} (72 \eta -180) \cos (u) e+\frac{1}{72} (144 \
\eta -360)\right)


==> include/radius-3.tex <==
\bigg(-665280 \eta ^2+1753920 \eta -1814400\bigg) e^6+\bigg(725760 \eta ^2-77490 \pi ^2 \eta +5523840 \eta -3628800\bigg) e^4+\bigg(544320 \eta ^2+154980 \pi ^2 \eta -14132160 \eta +7257600\bigg) e^2-604800 \eta ^2+6854400 \eta +\bigg(\bigg(302400 \eta ^2-1254960 \eta +453600\bigg) e^7+\bigg(-1542240 \eta ^2-38745 \pi ^2 \eta +6980400 \eta -453600\bigg) e^5+\bigg(2177280 \eta ^2+77490 \pi ^2 \eta -12373200 \eta +4989600\bigg) e^3+\bigg(-937440 \eta ^2-38745 \pi ^2 \eta +6647760 \eta -4989600\bigg) e\bigg) \cos (u)+\sqrt{1-e^2} \bigg(\bigg(-4480 \eta ^3-25200 \eta ^2+22680 \eta -120960\bigg) e^6+\bigg(13440 \eta ^3+4404960 \eta ^2+116235 \pi ^2 \eta -12718296 \eta +5261760\bigg) e^4+\bigg(-13440 \eta ^3+2242800 \eta ^2+348705 \pi ^2 \eta -19225080 \eta +16148160\bigg) e^2+4480 \eta ^3+45360 \eta ^2-8600904 \eta +\bigg(\bigg(-6860 \eta ^3+550620 \eta ^2-986580 \eta +120960\bigg) e^7+\bigg(20580 \eta ^3-2458260 \eta ^2+3458700 \eta -2358720\bigg) e^5+\bigg(-20580 \eta ^3-3539340 \eta ^2-116235 \pi ^2 \eta +20173860 \eta -16148160\bigg) e^3+\bigg(6860 \eta ^3-1220940 \eta ^2-464940 \pi ^2 \eta +17875620 \eta -4717440\bigg) e\bigg) \cos (u)+116235 \eta  \pi ^2+1814400\bigg)-77490 \eta  \pi ^2-1814400

==> include/radius-3a.tex <==
\left(-665280 \eta ^2+1753920 \eta -1814400\right) e^6-604800 \eta ^2+6854400 \eta -1814400

==> include/radius-3b.tex <==
e^4 \left(725760 \eta ^2-77490 \pi ^2 \eta +5523840 \eta -3628800\right)-77490 \eta  \pi ^2

==> include/radius-3c.tex <==
e^2 \left(544320 \eta ^2+154980 \pi ^2 \eta -14132160 \eta +7257600\right)

==> include/radius-3d.tex <==
\left(\left(302400 \eta ^2-1254960 \eta +453600\right) e^7+\left(-1542240 \eta ^2-38745 \pi ^2 \eta +6980400 \eta -453600\right) e^5+\left(2177280 \eta ^2+77490 \pi ^2 \eta -12373200 \eta +4989600\right) e^3+\left(-937440 \eta ^2-38745 \pi ^2 \eta +6647760 \eta -4989600\right) e\right) \cos (u)

==> include/radius-3d1.tex <==
\left(302400 \eta ^2-1254960 \eta +453600\right) e^7+\left(-1542240 \eta ^2-38745 \pi ^2 \eta +6980400 \eta -453600\right) e^5

==> include/radius-3d2.tex <==
e \left(-937440 \eta ^2-38745 \pi ^2 \eta +6647760 \eta -4989600\right)

==> include/radius-3d3.tex <==
e^3 \left(2177280 \eta ^2+77490 \pi ^2 \eta -12373200 \eta +4989600\right)

==> include/radius-3e.tex <==
\sqrt{1-e^2} \left(\left(-4480 \eta ^3-25200 \eta ^2+22680 \eta -120960\right) e^6+\left(13440 \eta ^3+4404960 \eta ^2+116235 \pi ^2 \eta -12718296 \eta +5261760\right) e^4+\left(-13440 \eta ^3+2242800 \eta ^2+348705 \pi ^2 \eta -19225080 \eta +16148160\right) e^2+4480 \eta ^3+45360 \eta ^2-8600904 \eta +\left(\left(-6860 \eta ^3+550620 \eta ^2-986580 \eta +120960\right) e^7+\left(20580 \eta ^3-2458260 \eta ^2+3458700 \eta -2358720\right) e^5+\left(-20580 \eta ^3-3539340 \eta ^2-116235 \pi ^2 \eta +20173860 \eta -16148160\right) e^3+\left(6860 \eta ^3-1220940 \eta ^2-464940 \pi ^2 \eta +17875620 \eta -4717440\right) e\right) \cos (u)+116235 \eta  \pi ^2+1814400\right)

==> include/radius-3e1.tex <==
\left(-4480 \eta ^3-25200 \eta ^2+22680 \eta -120960\right) e^6+4480 \eta ^3+45360 \eta ^2-8600904 \eta +1814400

==> include/radius-3e2.tex <==
\left(13440 \eta ^3+4404960 \eta ^2+116235 \pi ^2 \eta -12718296 \eta +5261760\right) e^4+116235 \eta  \pi ^2

==> include/radius-3e3.tex <==
e^4 \left(13440 \eta ^3+4404960 \eta ^2+116235 \pi ^2 \eta -12718296 \eta +5261760\right)

==> include/radius-3e4.tex <==
\left(-13440 \eta ^3+2242800 \eta ^2+348705 \pi ^2 \eta -19225080 \eta +16148160\right) e^2+\left(\left(-6860 \eta ^3+550620 \eta ^2-986580 \eta +120960\right) e^7+\left(20580 \eta ^3-2458260 \eta ^2+3458700 \eta -2358720\right) e^5+\left(-20580 \eta ^3-3539340 \eta ^2-116235 \pi ^2 \eta +20173860 \eta -16148160\right) e^3+\left(6860 \eta ^3-1220940 \eta ^2-464940 \pi ^2 \eta +17875620 \eta -4717440\right) e\right) \cos (u)

==> include/radius.tex <==
\frac{1-e \cos (u)}{x}+\left(\frac{2 (e \cos (u)-1)}{e^2-1}+\frac{1}{6} (2 \
(\eta -9)+e (7 \eta -6) \cos (u))\right)+\left(\frac{\left((26 \eta -51) \
e^2+28 \eta -48\right) (e \cos (u)-1)}{6 \left(e^2-1\right)^2}+\frac{72 (7 \
\eta -4)+36 \sqrt{1-e^2} (2 \eta -5) (e \cos (u)+2)+\left(1-e^2\right) \
\left(8 \eta ^2+30 \eta +e (7 (33-5 \eta ) \eta -72) \cos (u)+72\right)}{72 \
\left(1-e^2\right)}\right) x+\left(-\frac{\left(16 \left(\eta  \left(65 \
\sqrt{1-e^2} \eta -110 \sqrt{1-e^2}+96\right)+156 \sqrt{1-e^2}-240\right) \
e^4+\left(192 \left(87 \sqrt{1-e^2}+10\right)+\eta  \left(\sqrt{1-e^2} \
\left(5120 \eta +123 \pi ^2\right)-256 \left(86 \
\sqrt{1-e^2}+3\right)\right)\right) e^2+128 \left(-6 \eta +41 \
\sqrt{1-e^2}+15\right)+4 \sqrt{1-e^2} \eta  \left(224 \eta +123 \pi \
^2-4776\right)\right) (e \cos (u)-1)}{192 \left(1-e^2\right)^{7/2}}-\frac{72 \
(7 \eta -4)+36 \sqrt{1-e^2} (2 \eta -5) (e \cos (u)+2)+\left(1-e^2\right) \
\left(8 \eta ^2+30 \eta +e (7 (33-5 \eta ) \eta -72) \cos (u)+72\right)}{36 \
\left(e^2-1\right)^2}+\frac{\frac{(2 (\eta  (2 \eta  (8 \eta +45)-81)+432)+e \
(\eta  (\eta  (49 \eta -3933)+7047)-864) \cos (u)) e^4}{1296}+\left(-\frac{4 \
\eta ^3}{81}-\frac{341 \eta ^2}{18}+\left(\frac{2099}{35}-\frac{41 \pi \
^2}{64}\right) \eta +\frac{1}{648} e (\eta  ((3933-49 \eta ) \eta \
-7047)+864) \cos (u)-\frac{52}{3}\right) e^2+\frac{(\eta  (\eta  (49 \eta \
-3933)+7047)-864) \cos (u) e}{1296}+\frac{2 \eta ^3}{81}-\frac{151 \eta \
^2}{36}+\frac{56221 \eta }{840}+\frac{1}{576} \sqrt{1-e^2} \left(e \left(48 \
(\eta  (20 \eta -83)+30) e^2+\eta  \left(-2976 \eta -123 \pi \
^2+19952\right)-12960\right) \cos (u)-2 \left(96 (\eta  (11 \eta -29)+30) \
e^2+\eta  \left(960 \eta +123 \pi \
^2-13184\right)+8640\right)\right)-\frac{123 \eta  \pi \
^2}{64}-\frac{70}{3}}{\left(e^2-1\right)^2}\right) x^2+O\left(x^3\right)


==> include/xDot-2.tex <==
\big(1964256 \eta ^2-3259980 \eta +3523113\big) e^8+\big(64828848 \eta ^2-123108426 \eta +83424402\big) e^6+\big(16650606060 \eta ^2-207204264 \eta +783768\big) e^4+\big(61282032 \eta ^2+15464736 \eta -92846560\big) e^2+1903104 \eta ^2+\sqrt{1-e^2} \big((2646000-1058400 \eta ) e^6+(64532160-25812864 \eta ) e^2-580608 \eta +1451520\big)+4514976 \eta -360224
